Ripple sparse self-attention for monaural speech enhancement

The use of Transformer represents a recent success in speech enhancement. However, as its core component, self-attention suffers from quadratic complexity, which is computationally prohibited for long speech recordings. Moreover, it allows each time frame to attend to all time frames, neglecting the strong local correlations of speech signals. This study presents a simple yet effective sparse self-attention for speech enhancement, called ripple attention, which simultaneously performs fine- and coarse-grained modeling for local and global dependencies, respectively. Specifically, we employ local band attention to enable each frame to attend to its closest neighbor frames in a window at fine granularity, while employing dilated attention outside the window to model the global dependencies at a coarse granularity. We evaluate the efficacy of our ripple attention for speech enhancement on two commonly used training objectives. Extensive experimental results consistently confirm the superior performance of the ripple attention design over standard full self-attention, blockwise attention, and dual-path attention (Sep-Former) in terms of speech quality and intelligibility.

==> data/com.tex <==
\renewcommand\arraystretch{1.0}
\vspace{-1.0em}
\begin{table}[!hbpt]
\centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{2.3pt}
\caption{Average scores of CSIG, CBAK, and COVL across all test conditions. The highest scores are highlighted in boldface.}
\label{tabwer}
\vspace*{0.1in}
\scalebox{1}{
\begin{tabular}{l|ccc|ccc }
\toprule
\multirow{2}{*}{\textbf{Network}}  & \multicolumn{3}{c|}{\textbf{IRM}} & \multicolumn{3}{c}{\textbf{PSM}}  \\
\cline{2-7}
 &  \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} & \textbf{CSIG} & \textbf{CBAK} & \textbf{COVL} \\
\toprule 
Noisy & 2.26  & 1.80  & 1.67  & - & - & -  \\
\toprule   
% \textbf{GaResTCN}       
%  & 3.15 & 2.48 & 2.42 & 3.15 & 2.51 & 2.45 \\
ResTCN+SA \cite{restcnsa}     
& 3.10 & 2.45 & 2.37 & 3.14 & 2.53 & 2.46 \\
MHANet \cite{mhanet}      
& 3.13 & 2.46 & 2.40 & 3.21 & 2.56 & 2.51 \\
\toprule 
ResTCN \cite{deepmmse}     
& 3.08 & 2.43 & 2.35 & 3.12 & 2.52 & 2.44 \\
ResTCN+FA    
& 3.21 & 2.51 & 2.48 & 3.25 & 2.61 & 2.55 \\      
ResTCN+TA       
& 3.23 & 2.53 & 2.49 & 3.27 & 2.58 & 2.57 \\
ResTCN+TFA    
& \textbf{3.28} &\textbf{2.56} & \textbf{2.54} & \textbf{3.33} & \textbf{2.64} & \textbf{2.62} \\  
% \midrule[0.8pt]
% \midrule[0.8pt]
% ResMLP      & 2.60  & 2.14 & 1.95 & 2.64 & 2.18 & 2.00 \\
% ResMLP+TFA  & \textbf{2.95} & \textbf{2.31} & \textbf{2.23} & \textbf{2.95} & \textbf{2.39} & \textbf{2.28} \\
\toprule  
\end{tabular}}
\label{composite}
\vspace{-2em}
\end{table}

==> data/estoi.tex <==
\begin{table}[!htbp]
    % \vspace{-1.0em}
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{4.5pt}
    \footnotesize	
    \caption{Average ESTOI scores (in \%) for each SNR level. The highest ESTOI scores are highlighted in boldface.}
    \label{tabwer}
    \vspace{1.5in}
    \scalebox{0.90}{\begin{tabular}{clrccccc}
        \toprule
        & & & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cmidrule[0.8pt]{4-8}
        \textbf{Target} & \textbf{Network} & {\textbf{\# Params}} & -5 & 0 & 5 & 10 & 15 \\
        \toprule
        - & Noisy & & 27.91 & 42.14 & 57.21 & 71.11 & 82.22 \\
        \toprule
        \multirow{5}{*}{\textbf{IRM}}
        % & ResLSTM & 43.16 & 59.80 & 73.16 & 82.74 & 89.25  \\
        % & CRN & 43.97 & 61.27 & 74.40 & 83.39 & 89.55  \\
        % & GaResTCN   & 3.78M & 43.02 & 60.70 & 74.53 & 83.80 & 89.79  \\
        & ResTCN+SA \cite{restcnsa}    & 2.24M & 43.32 & 60.68 & 74.37 & 83.67 & 89.77  \\
        & MHANet \cite{mhanet}       & 4.08M & 43.72 & 61.08 & 74.68 & 83.90 & 89.96  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}       & 1.98M  & 42.47 & 59.93 & 73.67 & 83.22 & 89.44  \\
        & ResTCN+FA    & +1.36K & 44.87 & 61.73 & 75.06 & 84.27 & 90.09\\
        & ResTCN+TA    & +1.36K & 46.11 & 62.96 & 75.86 & 84.48 & 90.21\\
        & ResTCN+TFA   & +2.72K & \textbf{47.61} & \textbf{64.05} & \textbf{78.61} & \textbf{85.45} & \textbf{90.83}\\
        % \cmidrule[0.8pt]{2-8}
        % & ResMLP        & 1.58M  & 31.76 & 48.39 & 64.36 & 77.04 & 85.71 \\
        % & ResMLP+TFA    & +0.34K & \textbf{38.14} & \textbf{55.39} & \textbf{70.11} & \textbf{81.08} & \textbf{88.33} \\
        \toprule
        \toprule
        
        \multirow{5}{*}{\textbf{PSM}}
        % & ResLSTM & 42.73 & 60.11 & 74.02 & 83.55 & 89.84  \\
        % & CRN & 44.51 & 62.74 & 75.98 & 84.73 & 90.38  \\
        % & GaResTCN   & 3.78M & 42.77 & 60.75 & 74.58 & 84.05 & 90.01  \\
        & ResTCN+SA \cite{restcnsa}    & 2.24M & 43.03 & 61.13 & 75.07 & 84.24 & 90.07  \\
        & MHANet \cite{mhanet}       & 4.08M & 44.66 & 62.32 & 75.74 & 84.69 & 90.43  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}       & 1.98M  & 42.76 & 60.45 & 74.47 & 83.91 & 89.84  \\
        & ResTCN+FA    & +1.36K & 44.91 & 62.38 & 75.88 & 84.82 & 90.45\\
        & ResTCN+TA    & +1.36K & 45.70 & 63.25 & 76.49 & 85.09 & 90.70\\
        & ResTCN+TFA   & +2.72K & \textbf{48.67} & \textbf{65.28} & \textbf{77.43} & \textbf{85.80} & \textbf{91.16}\\

        \bottomrule
    \end{tabular}}
    \label{estoi}
    % \vspace{-0.5em}
\end{table}

==> data/pesq.tex <==
\begin{table}[!h]
    % \vspace{-1.0em}
    \centering
    \scriptsize
    \def\arraystretch{1.2}
    \setlength{\tabcolsep}{4.5pt}
    \footnotesize	
    \caption{Average PESQ (wideband version) scores for each SNR level. The highest PESQ scores are highlighted in boldface.}
    \label{tabwer}
    % \vspace*{0.5em}
    \scalebox{0.92}{\begin{tabular}{clrccccc}
        \toprule
        &  &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
        \cmidrule[0.8pt]{4-8}
        {\textbf{Target}} & {\textbf{Network}} & {\textbf{\# Params}} & -5 & 0 & 5 & 10 & 15 \\
        \toprule
        - & Noisy & & 1.05 & 1.07 & 1.13 & 1.31 & 1.64 \\
        \toprule
        \multirow{5}{*}{\textbf{IRM}}
        % &  GaResTCN \cite{grn}       & 3.78M & 1.15 & 1.36 & 1.68 & 2.12 & 2.58  \\
        & ResTCN+SA \cite{restcnsa} & 2.24M & 1.15 & 1.34 & 1.64 & 2.07 & 2.51  \\
        & MHANet \cite{mhanet}      & 4.08M & 1.16 & 1.36 & 1.68 & 2.10 & 2.56  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN 
        \cite{deepmmse} & 1.98M  & 1.13 & 1.32 & 1.61 & 2.06 & 2.50  \\
        & ResTCN+FA     & +1.36K & 1.18 & 1.39 & 1.74 & 2.15 & 2.60 \\
        & ResTCN+TA     & +1.36K & 1.18 & 1.40 & 1.75 & 2.19 & 2.63 \\
        & ResTCN+TFA    & +2.72K & \textbf{1.20} & \textbf{1.43} & \textbf{1.79} & \textbf{2.27} & \textbf{2.70}\\
        % \cmidrule[0.8pt]{2-8}
        % & ResMLP        & 1.58M  & 1.07 & 1.15 & 1.33 & 1.62 & 2.03 \\
        % & ResMLP+TFA    & +0.34K & \textbf{1.11} & \textbf{1.26} & \textbf{1.51} & \textbf{1.90} & \textbf{2.38} \\
        \toprule
        \toprule
        
        \multirow{5}{*}{\textbf{PSM}}
        % & GaResTCN \cite{grn}       & 3.78M & 1.18 & 1.41 & 1.77 & 2.24 & 2.72  \\
        & ResTCN+SA \cite{restcnsa} & 2.24M & 1.20 & 1.42 & 1.79 & 2.26 & 2.75  \\
        & MHANet \cite{mhanet}      & 4.08M & 1.20 & 1.44 & 1.83 & 2.30 & 2.78  \\
        \cmidrule[0.8pt]{2-8}
        & ResTCN \cite{deepmmse}    & 1.98M & 1.19 & 1.40 & 1.76 & 2.23 & 2.72  \\
        & ResTCN+FA   & +1.36K & 1.20 & 1.47 & 1.87 & 2.36 & 2.85\\
        & ResTCN+TA   & +1.36K & 1.21 & 1.49 & 1.90 & 2.38 & 2.85\\
        & ResTCN+TFA   & +2.72K & \textbf{1.26} & \textbf{1.54} & \textbf{1.96} & \textbf{2.44} & \textbf{2.91}\\
        \bottomrule
    \end{tabular}}
    \label{pesq}
    % \vspace{-1.5em}
\end{table}
